Measurement of the Spin of the Omega^- Hyperon at BABAR

A measurement of the spin of the Omega^- hyperon produced through the exclusive process Xi_c^0 --> Omega^- K^+ is presented using a total integrated luminosity of 116 fb^-1 recorded with the BABAR detector at the e^+ e^- asymmetric-energy B-Factory at SLAC. Under the assumption that the Xi_c^0 has spin 1/2, the angular distribution of the Lambda from Omega^- --> Lambda K^- decay is inconsistent with all half-integer Omega^- spin values other than 3/2. Lower statistics data for the process Omega_c^0 --> Omega^- pi^+ from a 230 fb^-1 sample are also found to be consistent with Omega^- spin 3/2. If the Xi_c^0 spin were 3/2, an Omega^- spin of 5/2 cannot be excluded.

==> minisym.tex <==
\RequirePackage{xspace}

\usepackage{relsize}

\def\babar{\mbox{\slshape B\kern-0.1em{\smaller A}\kern-0.1em
    B\kern-0.1em{\smaller A\kern-0.2em R}}}
\def\invfb   {\ensuremath{\mbox{\,fb}^{-1}}\xspace}
\def\ccbar {\ensuremath{c\overline c}\xspace}
\def\pep2{PEP-II}
\def\BB      {\ensuremath{B\Bbar}\xspace} 
\def\Bbar    {\kern 0.18em\overline{\kern -0.18em B}{}\xspace}

